3D Object Recognition with Ensemble Learning --- A Study of Point Cloud-Based Deep Learning Models

In this study, we present an analysis of model-based ensemble learning for 3D point-cloud object classification and detection. An ensemble of multiple model instances is known to outperform a single model instance, but there is little study of the topic of ensemble learning for 3D point clouds. First, an ensemble of multiple model instances trained on the same part of the $\textit{ModelNet40}$ dataset was tested for seven deep learning, point cloud-based classification algorithms: $\textit{PointNet}$, $\textit{PointNet++}$, $\textit{SO-Net}$, $\textit{KCNet}$, $\textit{DeepSets}$, $\textit{DGCNN}$, and $\textit{PointCNN}$. Second, the ensemble of different architectures was tested. Results of our experiments show that the tested ensemble learning methods improve over state-of-the-art on the $\textit{ModelNet40}$ dataset, from $92.65\%$ to $93.64\%$ for the ensemble of single architecture instances, $94.03\%$ for two different architectures, and $94.15\%$ for five different architectures. We show that the ensemble of two models with different architectures can be as effective as the ensemble of 10 models with the same architecture. Third, a study on classic bagging i.e. with different subsets used for training multiple model instances) was tested and sources of ensemble accuracy growth were investigated for best-performing architecture, i.e. $\textit{SO-Net}$. We also investigate the ensemble learning of $\textit{Frustum PointNet}$ approach in the task of 3D object detection, increasing the average precision of 3D box detection on the $\textit{KITTI}$ dataset from $63.1\%$ to $66.5\%$ using only three model instances. We measure the inference time of all 3D classification architectures on a $\textit{Nvidia Jetson TX2}$, a common embedded computer for mobile robots, to allude to the use of these models in real-life applications.

==> sections/3_8_best_test.tex <==
% %-------------------------------------------------------------------------
% \subsection{Model Selection Based on Best Test Result}
% \label{sec::test_overfit}

% The \textit{ModelNet40} dataset has a train and test split, without an explicit validation set. The question arises whether the mean or best test score should be reported. There are two hypotheses possible:
% \begin{enumerate}
%     \item The model instance is better than the other, so it should be selected.
%     \item The model instance can be over-fitted to the test data, so there is no reason to report its accuracy.
% \end{enumerate}
% Note that our experiments show that the reduction of training set size influences the overall accuracy, so selecting the validation set from the training samples would result in classification accuracy not comparable to ones reported in earlier studies. To verify this hypothesis, we split the test set into two parts and tested whether the best result on the first part correlates with a high result on the second one. To do this, we defined  the following:
% \begin{itemize}
%     \item average model instance result on a full test set $T$
%     \begin{equation}
%         acc_{mean}(T) = mean(acc_i(T), i = 1, \ldots, 10)
%     \end{equation}
%     \item maximum model instance result on a full test set $T$
%     \begin{equation}
%         acc_{max}(T) = max(acc_i(T), i = 1, \ldots, 10)
%     \end{equation}
%     \item full test set $T$ was split randomly $S = 1000$ times into two equal subsets: $A$ and $B$, we report the mean of maximum accuracy obtained on subset $A$:
%     %\item given $S = 1000$ splits of full test set $T$ into two equal subsets: $A$ and $B$, the mean of maximum accuracy obtained on subset $A$ by a single model:
%     \begin{equation}
%         \begin{split}
%         acc_{sel}(A) = & mean(max(acc_i(A_s), \\
%         & i = 1, \ldots, 10), s = 1, \ldots, S)
%         \end{split}
%     \end{equation}
%     %which will be equal to $acc_{max}$ when $S \rightarrow \infty$
%     \item given $S = 1000$ splits of full test set $T$ into two equal subsets $A$ and $B$, the mean of  accuracy obtained on subset $B$ by a model with maximum accuracy on subset $A$:
%     \begin{equation}
%         \begin{split}
%         acc_{sel}(B) = & mean(acc_j(B_s), \\
%         & acc_j(A_s) = max(acc_i(A_s), \\
%         & i = 1, \ldots, 10),\\
%         & s = 1, \ldots, S)
%         \end{split}
%     \end{equation}
% \end{itemize}

% If $acc_{sel}(B)$ is significantly higher than  $acc_{mean}(T)$, then hypothesis 1 is supported; otherwise hypothesis 2 is supported.

% \begin{table}[t]
% \renewcommand\thetable{1}
% \caption{Test of model instance selection based on the best test score. The test set was split randomly 1000 times; the best model was selected based on part A and then tested on part B. For each architecture, the value of $acc_{sel}(B)$ is lower than the value of $acc_{max}(T)$, which suggests that the selection of best training instance by its test results can lead to overfitting.}

% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccc}
% \hline \hline
%           & $acc_{mean}(T)$ & $acc_{max}(T)$ & $acc_{sel}(A)$ & $acc_{sel}(B)$ \\ \hline \hline
% \textit{PointNet}   & 88.65\%         & 89.06\%        & 89.24\%        & 88.59\%        \\
% \textit{PointNet++} & 90.14\%         & 90.64\%        & 90.79\%        & 90.33\%        \\
% \textit{DeepSets}   & 89.82\%         & 90.17\%        & 90.43\%        & 89.81\%        \\
% \textit{KCNet}      & 89.62\%         & 90.40\%        & 90.50\%        & 89.88\%        \\
% \textit{SO-Net}     & 92.65\%         & 92.95\%        & 93.19\%        & 92.46\%        \\ 
% \textit{DGCNN}      & 91.55\%         & 91.86\%        & 92.03\%        & 91.43\%        \\
% \textit{PointCNN}   & 91.82\%         & 91.98\%        & 92.22\%        & 91.63\%        \\
% Average    & 90.61\%         & 91.01\%        & 91.20\%        & 90.59\%        \\
% \hline \hline
% \end{tabular}}
% \label{tab::test_overfit}
% \end{table}

%Table \ref{tab::test_overfit} shows the results of model's instance selection. For each architecture, value of $acc_{sel}(B)$ is lower than the value of $acc_{max}(T)$ (mean difference $0.61\%$ ) and on an average slightly lower ($0.02\%$) than the value of $acc_{mean}(T)$. This supports the hypothesis that the selection of best training instance by its test results can lead to overfitting.
